Origins of Low-dimensional Adversarial Perturbations

In this paper, we initiate a rigorous study of the phenomenon of low-dimensional adversarial perturbations (LDAPs) in classification. Unlike the classical setting, these perturbations are limited to a subspace of dimension $k$ which is much smaller than the dimension $d$ of the feature space. The case $k=1$ corresponds to so-called universal adversarial perturbations (UAPs; Moosavi-Dezfooli et al., 2017). First, we consider binary classifiers under generic regularity conditions (including ReLU networks) and compute analytical lower-bounds for the fooling rate of any subspace. These bounds explicitly highlight the dependence of the fooling rate on the pointwise margin of the model (i.e., the ratio of the output to its $L_2$ norm of its gradient at a test point), and on the alignment of the given subspace with the gradients of the model w.r.t. inputs. Our results provide a rigorous explanation for the recent success of heuristic methods for efficiently generating low-dimensional adversarial perturbations. Finally, we show that if a decision-region is compact, then it admits a universal adversarial perturbation with $L_2$ norm which is $\sqrt{d}$ times smaller than the typical $L_2$ norm of a data point. Our theoretical results are confirmed by experiments on both synthetic and real data.

==> art.tex <==
% \section{Understanding the Art of Singular Vectors for neural networks}
% Consider a ReLU neural network $f:\mathbb R^d \to \mathbb R$, fully-trained or not, for binary classification. For a sample of $n$ iid data points $x_1,\ldots,x_n \in \mathbb R^d$, define a random $n \times d$ matrix $J$ with $i$th row $\nabla f(x_i)$. Let $v \in \mathbb R$ be the top eigenvector of the psd matrix $d \times d$ psd matrix $M := J^\top J/n$. It was empirically observed in \cite{singularart} that ...
% \lorem

% \lorem 


==> ballfgsm.tex <==
One computes $\nabla f(x) = -x$ and so the $L_2$-FGSM perturbation
vector forinput $x$ as $a_\varepsilon(x) = -\varepsilon \nabla f(x)/\|\nabla f(x)\| = \varepsilon x /\|x\|$,
where $\varepsilon \ge 0$ is the budget of the attacker. It is clear that $x+a_\varepsilon(x) \in C$ iff $1 \ge \|x+\varepsilon x/\|x\|\| = \|x\|+\varepsilon$. Thus, the subset of the feature space $\mathbb R^d$ on which the
classifier flips its decision from positive to negative, upon addition of the
perturbation $a_\varepsilon(x)$, is the annulus with inner radius $1-\varepsilon$ and outer
radius $1$, namely
% \begin{eqnarray}
$B_d^{-\varepsilon}
% := \{x \in
% \mathbb R^d \mid f(x+a_\varepsilon()) = -1,\; f(x) = 1\}
% = \{x \in \mathbb R^d \mid \|x\| \le 1 < \|x + (\varepsilon/\|x\|)x\|\}
= \inte(B_d) \setminus \varepsilon B_d = \{x \in \mathbb R^d \mid
  1-\varepsilon \le \|x\| < 1\}.
  $
% \end{eqnarray}

Let $\omega_d=\pi^{d/2}/\Gamma(d/2+1)$ be the volume of the unit sphere $B_d$. Then
$\omega_d-(1-\varepsilon)^d\omega_d \ge \omega_d(1-e^{-\varepsilon d})$ is the volume of the annulus $B_d^{-\varepsilon}$
and so the fooling rate of the FGSM attack on the positive class is
\begin{eqnarray}
  \label{eq:spherepinch}
  \begin{split}
  \mathbb P_X(X + a_\varepsilon(X) \in C\mid X \in C') &= \frac{\vol(B_d^{-\varepsilon})}{\vol(B_d)}
  \begin{cases}=1,&\mbox{ if }\varepsilon \ge 1,\\\ge 1-e^{-\varepsilon d},&\mbox{ if }0 \le \varepsilon < 1.\end{cases}
  \end{split}
\end{eqnarray}
Thus, taking $\varepsilon = 1/d$, we see that
at least a staggering $63\%$ of all the points of
the class $C$ are located at a distance $1/d$ from the decision boundary!\footnote{Since $1-1/e > 0.63$.}
% We note that the FGSM attack is optimal for this problem.


==> checklist.tex <==
\section*{Checklist}


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}: for each theorem, the conditions and hypothsesis under which they hold are clearly stated (see Conditions \ref{cond:strongslope}, \ref{cond:smooth}, \ref{cond:beta}, \ref{cond:almostconstgrad}, \ref{cond:bottleneck} in Sections \ref{sec:smooth} and \ref{sec:local})
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}, we don't expect any.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}, in Sections \ref{sec:smooth} and \ref{sec:local}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{} in the Appendix
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}, as explained in Section \ref{subsec:experiments}. The code is given in a separate zip file.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNo{}, as our experiments have illustration purposes and are very simple.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}, as our experiments are very quick even on a basic setup (personal computer, no specific ressources).
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}, as the MNIST dataset is widely used.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> objectives.tex <==
Our objective is to establish the existence of adversarial subspaces $V \subseteq \bR^d$ such that
% \begin{mdframed}
\begin{itemize}
\item \textit{The subspace is low-dimensional:} $\dim V = k = o(d)$, i.e. $k/d \to 0$ as $d \to \infty$.
\item\textit{The perturbations are small:} The (maximum) size of the allowed perturbations is $\varepsilon = o(r_X)$, i.e. $\varepsilon /r_X \to 0$, where $r_X := (\mathbb E\|X\|^2)^{1/2}$.
\item\textit{The fooling rate is high.} The fooling rate is bounded away from zero, i.e $\fr(V;\varepsilon) \ge c$ for some absolute constant $c>0$.
\end{itemize}

%  \lorem 

%\end{mdframed}
We shall obtain lower-bounds for the fooling rate $\fr(V;\varepsilon) := \bP(X \in C^{\varepsilon}_V \mid X \in C')$ in a variety of situations. In case the subspace $V$ is itself random, these lower-bounds will either be w.h.p. over $V$, or else we will simply lower-bound the expected fooling rate $\mathbb E_V[\fr(V;\varepsilon)]$.

==> polytope.tex <==
\section{Closed convex polytopes}
\mytodo{Reformulate the results of this section in terms of arbitrary isoperimetric profiles (not just gaussians)!}
Now, suppose the decision region $C$ is a non-empty intersection of a finite number of half-spaces in $\mathbb R^d$, i.e.,
\begin{eqnarray}
C = \cap_{i=1}^N H_i,\text{ with }H_i := \{x \in \mathbb R^d \mid x^\top w_i + b_i \le 0\},
\end{eqnarray}
where $w_1,\ldots,w_N$ are unit-vectors in $\mathbb R^d$ and $b_1,\ldots,b_N$ are scalars.

% \lorem
% It is a hallmark result of the % \emph{Bakry-\'Emery-Ledoux Theory (BELT)} of concentration that\footnote{E.g, see Theorem 1.2 of Bouyrie's manuscript on the subject \url{https://arxiv.org/abs/1708.07203}.}, the isoperimetric profile of $\mu$ is lower-bounded by $\sigma^2$ times that of $\gamma_1$, the standard gaussian distribution on $\mathbb R^1$. \mytodo{Missing citation!}
% \begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}{thm}{polytope}
% Let $X$ be a random vector in $\mathbb R^d$ with $\sigma^2$-log-concave isotropic distribution.
% Let $1 \le k \le d$ and let $V$ be drawn from the Haar measure on the grassmannian $\mathcal G_{k,d}$. Let $C$ be a (nonempty) convex subset of $\mathbb R^d$.
For any subspace $V$ of $\mathbb R^d$, define $\alpha_V(C) \in [0,1]$ by
\begin{eqnarray}
\alpha_V(C) := \min_{i \in [N]}\alpha_V(H_i) = \min_{i \in [N]}\|\Pi_Vw_i\|.
\end{eqnarray}
Then, for any $\varepsilon \ge 0$, it holds that
\begin{eqnarray}
\label{eq:convset}
\mathbb P_X(X \in C^\varepsilon_V) \ge J_X(p,\alpha_V(C)\sigma^2\varepsilon),
\end{eqnarray}
where $p=\mathbb P(X \in C)$.
Moreover, the lower-bound \eqref{eq:convset} is tight: it is attained when $X$ Gaussian distribution with covariance $\sigma^2 $ and $C$ is half-space.
\label{thm:polytope}
\end{restatable}
%\end{mdframed}
The result is proved by first establishing that $C^{\varepsilon'} \subseteq C^\varepsilon_V$, where $\varepsilon' := \alpha_V(C)$. The rest of the proof then lower-bounds $\bP_X(X \in C^{\varepsilon}_V)$ via a basic computation to get the RHS of \eqref{eq:convset}. The full proof is provided in the appendix.

% The result is proved in Section \ref{sec:proofs}.
The following corollary is just as important ...
%\begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}{cor}{}
Let $V$ be a uniformly-random $k$-dimensional subspace of $\mathbb R^d$. Let $C$ be as in Theorem \ref{thm:polytope}, with the restriction that the number of half-spaces $N$ is strictly subexponential in $k$ (e.g., polynomial), i.e., $(1/k)\log N \to 0$. Then, for any $\varepsilon \ge 0$ and $t \in (0,\sqrt{k/d})$ it holds w.p. $1-e^{-t^2d/2}$ over $V$ that
\begin{eqnarray}
\label{eq:randV}
\mathbb P(X \in C^\varepsilon_V) \ge J_X(p,(\sqrt{k/d}-t)\sigma^2 \varepsilon),
\end{eqnarray}
where $p:=\mathbb P(X \in C)$ as usual.
\label{cor:randV}
\end{restatable}
% \end{mdframed}
\begin{proof}%[Proof of Corollary \ref{cor:randV}]
For each $i \in [N]$, we know from \eqref{eq:concentrateThetaH} that the quantity $\alpha_V(H_i)^2 = \|\Pi_Vw_i\|^2 = w_i^\top \Pi_Vw_i$ has Gaussian concentration around its expected value of $\mathbb E_V[\mbox{trace}(P_V)] = k/d$. It then follows from a basic union bound (since $N$ is strictly subexponential in $k$) that for any $s \in (0,\sqrt{k/d})$, it holds w.p. $1-o_d(1)$ over $V$ that $\alpha_V(C) = \min_{i \in [N]}\alpha_V(H_i) \ge \sqrt{k/d}-t$. The claim then follows from Theorem \ref{thm:polytope}.
\end{proof}

==> polytope_proof.tex <==
\subsection{Proof of Theorem \ref{thm:polytope}}
\polytope*

We will need the following auxiliary lemma.
\begin{restatable}{lm}{}
\label{lm:alphaV}
Let $C := \cap_{i=1}^N H_i$, $V$, and $\alpha_V(C)$ be as in Theorem \ref{thm:polytope}.
Then, we have
\begin{eqnarray}
C^{\alpha_V(C)\varepsilon} \subseteq C^\varepsilon_V.
\end{eqnarray}
\end{restatable}

\begin{proof}
If $\varepsilon = 0$, both sets are equal to $C$ and there is nothing to prove. Otherwise, let $x \in C^{\alpha_V(C)\varepsilon}$, where $C^\delta$ is the usual $\delta$-expansion of $C$. Then, $\mbox{dist}(x, C) \le \alpha_V(C) \varepsilon$. Now, it is an elementary result that the distance from a point to the intersection of a collection of sets is at least equal to the largest distance between the point and any of the sets.
% \footnote{Indeed $\dist(x,\cap H_i) := \inf_{x' \in \cap_i H_i}\|x-x'\| \ge \|x-x'\|$ for all $i$, and so $\dist(x,\cap H_i) \ge \sup_i \dist(x,H_i)$.}.
Using this fact, one computes
\begin{eqnarray}
\begin{split}
\frac{1}{\varepsilon}\cdot\max_{i \in [N]}(x^\top w_i-b_i)_+ &= \frac{1}{\varepsilon}\cdot \max_{i \in [N]} \mathrm{dist}(x,H_i) \le \frac{\mbox{dist}(x, C)}{\varepsilon}\\
&\le \alpha_V(C) := \min_{i \in [N]}\|P_Vw_i\|\\
&= \min_{i \in [N]}\sup_{v \in V \cap B_d}v^\top w_i\\
&= \sup_{v \in V \cap B_d}\min_{i \in [N]}v^\top w_i.
\end{split}
\end{eqnarray}
Thus, there exists $v \in V \cap B_d$ such that $x^\top w_i - b_i \le \varepsilon v^\top w_i$, i.e $(x-\varepsilon v)^\top w_i \le b_i$ for all $i \in [N]$. We conclude that $x \in C^\varepsilon_V$.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:polytope}]
% It's not a loss of generality to assume that $C$ is closed.
% We provide a complete solution for the case where $C$ is the intersection of $N = \mathcal O(\mathrm{poly}(n))$ half-spaces $H_i := \{x \in \mathbb R^d \mid x^\top w_i \le b_i\}$, where each $w_i$ is a unit-vector in $\mathbb R^d$ and $b_i \in \mathbb R$.
Let $p:=\mathbb P(X \in C)$. By the definition of the isoperimetric profile $I_X$ of $X$, we have
%Since $X$ has Gaussian concentration, we have
\begin{eqnarray}
\mathbb P_X(0 < d_C(X) \le \varepsilon) \ge I_X(p)%\sigma^2 g(p)
\text{ for }\varepsilon \to 0^+.
\label{eq:iso}
\end{eqnarray}
% where $I_X$ is the isoperimetric profile of data $X$.
% g(p):= \dfrac{{\rm d}}{{\rm}d\varepsilon}\Phi(\Phi^{-1}(p)+\varepsilon)\bigg|_{\varepsilon=0} = \varphi(\Phi^{-1}(p))$ is the Gaussian \emph{isoperimetric profile}.
On the other hand, we know by virtue of Lemma \ref{lm:alphaV} that $C^{\varepsilon'} \subseteq C_V^\varepsilon$ where $\varepsilon' := \alpha_V(X)\varepsilon$, and so
\begin{eqnarray}
\begin{split}
\mathbb P_X(X \in C^\varepsilon_V ) - \bP_X(X \in C) &\ge \mathbb P_X(X \in C^{\varepsilon'}) - \bP_X(X \in C)\\
&= \int_0^{\varepsilon'} \mathbb P(d_C(X) \in {\rm d}\delta)\\
&\ge \int_0^{\varepsilon'} I_X(p){\rm d}\delta(1+o_\varepsilon(1))\\
&= I_X(p)(1+o_\varepsilon(1))\varepsilon'\\
&= \alpha_V(C)I_X(p)(1+o_\varepsilon(1))\varepsilon\\
\end{split}
\end{eqnarray}
Dividing through by $\varepsilon$ and taking $\varepsilon \to 0^+$ then gives
$$
\liminf_{\varepsilon \to 0^+}\frac{\mathbb P_X(X \in C^\varepsilon_V ) - \bP_X(X \in C)}{\varepsilon} \ge \alpha_V(C)I_X(p).
% = \alpha_V(C)\varphi(\Phi^{-1}(p)).
$$
Integrating w.r.t. $\varepsilon$ then gives the desired result.

\emph{Tightness.} Indeed, there is equality in \eqref{eq:convset} when $C$ is a half-space because in that case, \eqref{eq:iso} is an equality.
\end{proof}
